MCMARL: Parameterizing Value Function via Mixture of Categorical Distributions for Multi-Agent Reinforcement Learning

In cooperative multi-agent tasks, a team of agents jointly interact with an environment by taking actions, receiving a team reward and observing the next state. During the interactions, the uncertainty of environment and reward will inevitably induce stochasticity in the long-term returns and the randomness can be exacerbated with the increasing number of agents. However, such randomness is ignored by most of the existing value-based multi-agent reinforcement learning (MARL) methods, which only model the expectation of Q-value for both individual agents and the team. Compared to using the expectations of the long-term returns, it is preferable to directly model the stochasticity by estimating the returns through distributions. With this motivation, this work proposes a novel value-based MARL framework from a distributional perspective, \emph{i.e.}, parameterizing value function via \underline{M}ixture of \underline{C}ategorical distributions for MARL. Specifically, we model both individual Q-values and global Q-value with categorical distribution. To integrate categorical distributions, we define five basic operations on the distribution, which allow the generalization of expected value function factorization methods (\emph{e.g.}, VDN and QMIX) to their MCMARL variants. We further prove that our MCMARL framework satisfies \emph{Distributional-Individual-Global-Max} (DIGM) principle with respect to the expectation of distribution, which guarantees the consistency between joint and individual greedy action selections in the global Q-value and individual Q-values. Empirically, we evaluate MCMARL on both a stochastic matrix game and a challenging set of StarCraft II micromanagement tasks, showing the efficacy of our framework.

==> main_body_new.tex <==
\section{Methodology}

\begin{figure*}[htbp]
	\centering
	\subfigure[Lumberjacks]{
		\begin{minipage}{0.25\textwidth}%[b]%{0.2\textwidth}
			\includegraphics[width=\textwidth]{imgs/grid_world/Lumber.pdf}
		\end{minipage}
	}
	\hspace{0.9cm}
	\subfigure[TrafficJunction10]{
		\begin{minipage}{0.25\textwidth} 
            \includegraphics[width=\textwidth]{imgs/grid_world/Traffic10.pdf} 
		\end{minipage}
	}
	\hspace{0.9cm}
	\subfigure[SMAC]{
		\begin{minipage}{0.25\textwidth}%[b]%{0.2\textwidth}
			\includegraphics[width=\textwidth]{imgs/smac/smac.jpg}
		\end{minipage}
	}
	\caption{Visualisation of the three experimental environments.} 
	\label{grid_world}
\end{figure*}
In this section, we propose two strategies to investigate the discriminability of credit assignment in mixing network, \emph{i.e.}, an evaluation metric for discriminability measurement and a simplified version of QMIX.
Moreover, we design a gradient entropy regularization to enhance the discriminability of credit assignment.

\subsection{Discriminability Measurement of Credit Assignment via Gradient Entropy}
\label{measurement}
In this section, we propose an evaluation metric to measure the discriminability of credit assignment, and explain the rationale behind it.
Moreover, we employ this metric to evaluate the discriminability of credit assignment in QMIX.

Value decomposition paradigm approximates the global Q-value $Q_{tot}$ by the integration of a set of individual Q-values $Q_i$.
According to Taylor expansion, $Q_{tot}$ can be factorized as follows:
\begin{equation}
    \label{taylor}
    \begin{aligned}
    Q_{tot}&=Q_{tot}^0+(\frac{\partial Q_{tot}}{\partial \pmb{Q}})^T\pmb{Q}+o(\pmb{Q}^T\pmb{Q}) \\
    &\approx Q_{tot}^0+[g_1,\dots,g_n]^T\pmb{Q},
    \end{aligned}
\end{equation}
where $g_i$ denotes the gradient of $Q_{tot}$ over $Q_i$.
The above equation indicates that the influence of each agent on $Q_{tot}$ is determined by the corresponding gradient.
Moreover, a larger gradient means that the corresponding agent has a greater impact on $Q_{tot}$.

Considering that the gradient reflects each agent's contribution to the team, if the credits assigned to agents are discriminative, the gradient distribution over agents is unlikely to be uniform. To describe such non-uniformity, since the gradients are non-negative, we normalize them by Eq.~\eqref{normal} and adopt the entropy of the normalized gradients as a measure of the discriminability of credits assigned to agents.
\begin{equation}
    \label{normal}
    g_i^\prime=\frac{g_i}{\sum_{j=1}^n g_j}
\end{equation}
Beyond that, considering different complexity across tasks, we also normalize the entropy with the maximum entropy of $n$ random variables.
Based on the above discussion, the normalized gradient entropy is calculated as follows:
\begin{equation}
    \label{entropy}
    H_{norm}(\frac{\partial Q_{tot}}{\partial \pmb{Q}})=(-\sum_{i=1}^n g_i^\prime \log g_i^\prime)/\log n,
\end{equation}
where $\log n$ is the maximum entropy of $n$ values.
It can be seen that the smaller the entropy, the more discriminative the gradient, and vice versa.
In other words, if the normalized gradient entropy is close to 1, the gradients of $Q_{tot}$ on $\{ Q_i \}$ will be similar, meaning a lack of discriminability in credit assignment.

Given the definition of normalized gradient entropy, we employ it to measure the discriminability of credits assigned by QMIX.
It is worth noting that the normalized gradient entropy is applicable to measure the discriminability of any differentiable mixing network structure.
According to the mixing network structure in QMIX, the gradients of $Q_{tot}$ over $\{Q_i\}$ are calculated as follows:
\begin{equation}
    \label{gradient}
    [g_1,\dots,g_n]^T = \frac{\partial Q_{tot}}{\partial \pmb{Q}}=W_1^T F W_2,
\end{equation}
where $F=diag\{ \frac{df_{elu}(x)}{dx}|_{x=x_1}, \cdots, \frac{df_{elu}(x)}{dx}|_{x=x_n} \}$ is the gradient on the activation function $f_{elu}$. 
$x_i$ here is the $i$-th element in the output of the first linear layer in mixing network. 
As shown in Eq.~\eqref{qmix nonnegative}, each element of the gradient vector is non-negative.
The detailed derivation process can be found in supplementary material.

\subsection{Simplified QMIX}
\label{qsimple}

\begin{figure}[htb]
	\centering
	\subfigure{
		\begin{minipage}{0.6\textwidth}
          \includegraphics[width=\textwidth]{imgs/qsimple.pdf} 
		\end{minipage}
	}
	\caption{Simplified QMIX framework.
	Different from original QMIX, the simplified QMIX directly take the summation of individual $Q_i$s rather than $Q_i$ vector as the input of the mixing network.
	The parameters $W_1$ and $W_2$ produced by hypernetwork are scalars, compared to matrix in QMIX.} 
	\label{qsimple_framework}
\end{figure}

\begin{figure*}[htb]
    
	\centering
	\subfigure[Lumberjacks]{
	    \label{qmix_entropy_curve_Lumber}
		\begin{minipage}{0.3\textwidth}
            \includegraphics[width=\textwidth]{imgs/grid_world/entropy/Lumber_entropy.pdf}
		\end{minipage}
	}
	\subfigure[TrafficJunction10]{
	    \label{qmix_entropy_curve_Traffic10}
		\begin{minipage}{0.3\textwidth}
            \includegraphics[width=\textwidth]{imgs/grid_world/entropy/Traffic10_entropy.pdf}
		\end{minipage}
	}
	\\
	\resizebox{0.9\linewidth}{!}{\subfigure[3s5z]{
	    \label{qmix_entropy_curve_3s_vs_5z}
		\begin{minipage}{0.3\textwidth}
            \includegraphics[width=\textwidth]{imgs/smac/entropy_curve/3s5z_curve.pdf}
		\end{minipage}
	}
	\subfigure[MMM2]{
	    \label{qmix_entropy_curve_3s5z}
		\begin{minipage}{0.3\textwidth}
            \includegraphics[width=\textwidth]{imgs/smac/entropy_curve/MMM2_curve.pdf}
		\end{minipage}
	}
	\subfigure[27m vs 30m]{
	    \label{qmix_entropy_curve_27m_vs_30m}
		\begin{minipage}{0.3\textwidth}
            \includegraphics[width=\textwidth]{imgs/smac/entropy_curve/27m_vs_30m_curve.pdf}
		\end{minipage}
	}}
	\caption{Entropy curve during QMIX training (with y-axis ranging from 0.9 to 1.0).
	In (a) \emph{Lumberjacks} and (b) \emph{TrafficJunction10}, the data is collected as batch mean of normalized entropy every 1k steps.
	In (c) \emph{3s5z}, (d) \emph{MMM2} and (e) \emph{27m vs 30m} from SMAC, the data is collected every 10k steps.
	The solid line here shows the mean of the normalized entropy on five different random seeds.
	The upper and lower bound of shadow area represents the min and max entropy among 5 different random seeds.
	In these environments, the entropy keeps close to the maximum value (1.0) during the whole process except at the random exploration part, which means that the mixing network tends to assign equal credits to all the agents.} 
	\label{qmix_entropy_curve}
\end{figure*}
In addition to the discriminability measurement via gradient entropy, we conduct the ablation study to test the discriminability of QMIX in credit assignment.
To this end, we propose a simplified version of QMIX, named QMIX-simple, as a baseline.

QMIX-simple follows a similar paradigm as QMIX but simplifies the mixing strategy.
The overall framework of QMIX-simple is shown in Figure~\ref{qsimple_framework}.
Different from QMIX that integrates individual Q-values via learnable non-negative weights, QMIX-simple applies the summation operation over individual Q-values, followed by two scalar multiplications with an activation function in between.
Specifically, $Q_{tot}$ of QMIX-simple, denoted as $Q_{tot}^{simple}$, is calculated with the following equation:
% $Q_{tot}^{simple}$ here can be calculated with following equation:
\begin{equation}
    \label{qmix simple}
    Q_{tot}^{simple}=w_2 f_{elu}(w_1 (\sum_{i=1}^n Q_i)+b_1)+b_2,
\end{equation}
where $w_1 \in \mathbb{R}_+$, $w_2 \in \mathbb{R}_+$, $b_1 \in \mathbb{R}$ and $b_2 \in \mathbb{R}$ are produced by hypernetworks that take the global state as input.
% Different from $Q_{tot}$ in QMIX, the hyper parameters $w_1 \in \mathbb{R}_+$, $w_2 \in \mathbb{R}_+$, $b_1 \in \mathbb{R}$ and $b_2 \in \mathbb{R}$ are not matrix anymore, but are rather scalars. 
In this way, the gradients on $Q_i$ are forced to be equal and credits are assigned equally.

\begin{table}[htbp]
    \centering
    \resizebox{0.6\linewidth}{!} {
    \begin{tabular}{c|c|c}
        \hline
        Model & Equal Credits & Utilization of Global State \\
        \hline
        \textbf{VDN} & $\surd$ & $\times$ \\ 
        \textbf{QMIX} & $\times$ & $\surd$ \\ 
        \textbf{QMIX-simple} & $\surd$ & $\surd$ \\ 
        \hline
    \end{tabular}
    }
    \caption{Comparisons of three models.}
    \label{tab:model_diff}
\end{table}

\textbf{Discussion:} 
Here, we give a brief discussion of QMIX-simple, QMIX and VDN.
Table~\ref{tab:model_diff} summarizes the comparison of these three models.
% In addition to the difference between QMIX and QMIX-simple, it is worth discussing the difference between QMIX-simple and VDN as well.
VDN takes the sum of individual Q-values to approximate the global Q-value, which also assigns equal weights to agents.
The key difference between VDN and QMIX-simple is that QMIX-simple employs scalar multiplications and non-linear activation function to enrich the expressiveness of mixing network.
Besides, QMIX-simple takes the advantage of global state to get a state-dependent multiplicator while VDN actually ignores the global state.
Compared to QMIX, QMIX-simple also utilizes the global state in mixing network but explicitly assigns equal weights.
If QMIX-simple could achieve comparable performance as QMIX, it means that QMIX lacks discriminability in credit assignment.


\subsection{Gradient Entropy Regularization}
In this section, we propose a new method to guide QMIX to allocate different credits to different agents, named Gradient entropy REgularization (GRE).

In Section~\ref{measurement}, we have explained the rationality of employing gradient entropy to measure the discriminability of credit assignment.
Thereby, one straightforward way to enhance the discriminability of credit assignment is to incorporate the gradient entropy regularization into QMIX.
The overall loss of QMIX-GRE is the combination of the original TD loss and the regularizatioin term, \emph{i.e},
\begin{equation}
    \begin{aligned}
    \mathbb{L}&=\mathbb{L}_{TD_{loss}} + \lambda\mathbb{L}_{Reg}\\%\sum_{i=1}^b(\mathbb{L}_i^1+\mathbb{L}_i^2) \\
    &=\sum_{i=1}^b[(y_i^{tot}-Q_{tot}(\pmb{\tau},\pmb{u},s;\theta))^2+ \lambda H_{norm}(\frac{\partial Q_{tot}}{\partial \pmb{Q}})],
    \end{aligned}
    \label{reg}
\end{equation}
where $\lambda$ is a hyperparameter balancing the TD loss and the regularization term.
Note that when $\lambda = 0$, the model degenerates to the original QMIX.
A larger value of $\lambda$ means greater penalty for indiscriminability.
% where $\mathbb{L}_i^2=H_{norm}(\frac{\partial Q_{tot}}{\partial \pmb{Q}})$ term only updates the mixing network and $\lambda$ is a hyper parameter.
It is worth mentioning that optimizing the regularization term only updates the parameters in the mixing network.

\begin{table*}[htbp]
\centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{c|ccccc}
\hline
\diagbox{Percentile}{Env} & Lumberjacks & TrafficJunction10 & 3s5z & MMM2  & 27m vs 30m \\ \hline
5\%        & 0.972       & 0.931             & 0.941    & 0.961 & 0.987      \\
25\%       & 0.992       & 0.961             & 0.975    & 0.980 & 0.992      \\
50\%       & 0.997       & 0.975             & 0.984    & 0.988 & 0.995      \\
75\%       & 0.999       & 0.985             & 0.989    & 0.993 & 0.997      \\
95\%       & 1.000       & 0.993             & 0.995    & 0.996 & 0.999     \\ \hline
\end{tabular}}
\caption{The percentiles of gradient entropy of QMIX.
The data is collected during the whole training process and sorted from smallest to largest.
$i^{th}$ percentile value represents the $i\%$ smallest value in the data.
In all our experimental environments, the $25^{th}$ percentile of gradient entropy value is close to 1.
Since the maximum entropy means equal probability, the results here reveals the limited discriminablity of credit assignment in QMIX.}
\label{qmix_entropy_quantile}
\end{table*}

In our training process, the neural networks will minimize the TD loss as well as the normalized gradient entropy of the mixing network, forcing itself to assign different credits to different agents in an explicit way.
As a result, the mixing network will learn a more discriminative assignment mechanism.

\section{Experiments}
To comprehensively understand the credit assignment in QMIX and evaluate our proposed gradient entropy regularization, we conduct the experiments to answer the following questions in Section 5.2, 5.3, and 5.4, respectively:

\textbf{RQ1}: Does QMIX achieve a discriminative credit assignment via mixing network?

\textbf{RQ2}: With the help of gradient entropy regularization, how does QMIX-GRE perform compared to QMIX?

\textbf{RQ3}: Can QMIX-GRE enhance the discriminability of credit assignment?

\subsection{Experimental Settings}
In this section, we briefly introduce the experimental environments and the hyperparameter settings.
% In this paper, we conduct experiments on SMAC and several gridworld environments.

In this paper, we conduct experiments on two gridworld environments and SMAC environments.
The two gridworld environments, named Lumberjacks and TrafficJunction10, come from ~\cite{magym}.
SMAC is introduced by ~\cite{samvelyan19smac}

\textbf{Lumberjacks:}
The agents are lumberjacks whose goal is to cut down all the trees in the map. 
Each tree has a specified strength when an episode starts. 
For a tree in the map, once the number of agents in the cell of the tree is the same as or greater than its strength, the tree is automatically cut down. 
If all of the trees are cut down or the limit of the maximum episode step is reached, current episode ends.
The possible actions of agents are moving in four directions (Down, Left, Upper, Right) or do nothing.

\textbf{TrafficJunction10:}
The map is a 14 × 14 grid intersection and in each episode, there are 10 vehicles in total waiting to get into this intersection.
At each time step, ``new" cars enter the intersection from each of the four directions with probability $p$ and is randomly assigned to one of three possible routes (go straight, turn left and turn right).
Once a car reaches the edge of the grid, it will be removed. 
The total number of cars in the map at same time is limited. 
Cars are requested to keep on the right side of the road.
The car has two possible actions: move forward to its target or stay at the current cell. 
If the positions of two cars overlap, they collide and get a team reward -10, but this will not affect the simulation.
The reward of any time step is the sum of passed time steps of all the cars in the map with a negative factor and the collide reward.

\textbf{SMAC:}
This environment is built on Blizzard's StarCraft II RTS game and is very popular in MARL research field.
There are many maps in the environment where two teams of different agents try their best to defeat each other.
In the game, agents have no access to the global state and the observations are strictly limited.
In different maps of SMAC, the number and type of agents are different.
The actions of agents also depend on the scenario, whose number ranges from 7 to 70.
Once all the agents in a team die, the other team wins the game.
Although the overall target is to have the highest win rate for each scenario, the environment still offers a reward signal to help training.
This reward signal consists of hit-point damage dealt and received by agents, the units killed and the battle result.
% In the challenging tasks of SMAC, the agents need to highly cooperate with each other to protect themselves and defeat enemies.

Our implementation is based on PyMARL~\cite{samvelyan19smac} codebase and follows its hyperparameter settings. 
All the experiments in this paper are repeated five times with different random seeds.
The models are trained with 2M steps and tested every 10K steps in SMAC while trained with 200K steps and tested every 5K steps in other two environments.
Our codes are available in \url{https://github.com/sgzZ123/GRE}.

\begin{figure*}[htb]
	\centering
	\subfigure[Lumberjacks]{
		\begin{minipage}{0.25\textwidth}%[b]%{0.2\textwidth}
			\includegraphics[width=\textwidth]{imgs/grid_world/Lumber_simple.pdf}
		\end{minipage}
	}
	\subfigure[TrafficJunction10]{
		\begin{minipage}{0.25\textwidth}%[b]%{0.2\textwidth}
			\includegraphics[width=\textwidth]{imgs/grid_world/Traffic10_simple.pdf}
		\end{minipage}
	}
	\\
	\resizebox{0.8\linewidth}{!}{
	\subfigure[3s5z]{
		\begin{minipage}{0.3\textwidth}%[b]%{0.2\textwidth}
			\includegraphics[width=\textwidth]{imgs/smac/qsimple/qmix_simple_3s5z.pdf}
		\end{minipage}
	}
	\subfigure[MMM2]{
		\begin{minipage}{0.3\textwidth} 
            \includegraphics[width=\textwidth]{imgs/smac/qsimple/qmix_simple_MMM2.pdf} 
		\end{minipage}
	}
	\subfigure[27m vs 30m]{
		\begin{minipage}{0.3\textwidth}%[b]%{0.2\textwidth}
			\includegraphics[width=\textwidth]{imgs/smac/qsimple/qmix_simple_27m_vs_30m.pdf} 
		\end{minipage}
	}}
	\caption{The performance of QMIX and QMIX-simple.
	Both of the solid line are the mean performance from 5 different random seeds.
	The upper and lower bound of the shadow area are min and max values in the 5 seeds.
	(a) Lumberjacks and (b) TrafficJunction10 are experiments on gridworld, where QMIX-simple performs the same as QMIX.
	(c) \emph{3s5z}, (d) \emph{MMM2} and (e) \emph{27m vs 30m} are experiments on SMAC.
	In (c), the performance of QMIX-simple is close to the performance of QMIX, although with a tiny drop which probably comes from the decrease of parameters.
	In (d), QMIX-simple even outperforms the original QMIX.
	In (e) QMIX-simple performs the same as original QMIX.
	} 
	\label{qsimple_performance}
\end{figure*}
\subsection{Investigation of QMIX: RQ1}

To evaluate the discriminability of credits assigned by QMIX, we employ the normalized gradient entropy metric and compare the performance of QMIX and QMIX-simple.

To calculate the normalized gradient entropy, we collect the normalized entropy data on various SMAC environments and gridworld environments.
Table~\ref{qmix_entropy_quantile} summarizes the $q^{th}$ ($q \in \{5,25,50,75,95\}$) percentile of entropy values for each map/environment, respectively.
Across the five experimental environments, the differences between the $95^{th}$ and $5^{th}$ percentile of entropy values are small, which indicate that the gradient entropy in QMIX consistently follows a long-tail distribution.
Figure~\ref{qmix_entropy_curve} shows the normalized entropy curve in training process, where the y-axis ranges from 0.9 to 1.0.
We can find the normalized entropy keeps close to the maximal value except for random exploration stage where agents randomly select their actions.
To sum up, the distribution of gradient entropy demonstrates that QMIX suffers discriminability issue on the assignment of credits to agents.

In addition to discriminability measurement via gradient entropy, we conduct the ablation study to test the discriminability of QMIX in credit assignment.
We conduct experiments on various SMAC environments and gridworld environments.
In practice, we change the output of hypernetworks from matrix to scalars and keep other hyperparameters the same as original QMIX.
% Some of the results are plotted as figure \ref{qsimple_performance} shows and the results confirm our proposals.
Due to the page limit, we show the performance of QMIX-simple and QMIX on five representative maps/environments in Figure~\ref{qsimple_performance}.
The results on the remaining five maps of SMAC environments can be found in appendix.
We can find that the performance of QMIX-simple is extremely close to the original QMIX algorithm except for few environments with only a minor drop.
The performance drop probably comes from the decrease in the number of hypernetwork parameters (from matrices to scalars).

In summary, both the large value of gradient entropy and comparable performance of QMIX-simple to QMIX demonstrate that the credit assignment in QMIX still lacks discriminability. 

\subsection{Comparative Results: RQ2}
\begin{figure*}[htbp]
	\centering
	\subfigure[Lumberjacks]{
		\begin{minipage}{0.25\textwidth} 
            \includegraphics[width=\textwidth]{imgs/grid_world/regd/Lumber_reg0001.pdf}
		\end{minipage}
	}
	\subfigure[TrafficJunction10]{
		\begin{minipage}{0.25\textwidth} 
            \includegraphics[width=\textwidth]{imgs/grid_world/regd/Traffic10_reg01.pdf}
		\end{minipage}
	}
	\\
	\resizebox{0.8\linewidth}{!}{
	\subfigure[3s5z]{
		\begin{minipage}{0.3\textwidth} 
            \includegraphics[width=\textwidth]{imgs/smac/regd/qmix_regd0001_3s5z.pdf} 
		\end{minipage}
	}
	\subfigure[MMM2]{
		\begin{minipage}{0.3\textwidth} 
            \includegraphics[width=\textwidth]{imgs/smac/regd/qmix_regd0001_MMM2.pdf}
		\end{minipage}
	}
	\subfigure[27m vs 30m]{
		\begin{minipage}{0.3\textwidth}%[b]%{0.2\textwidth}
			\includegraphics[width=\textwidth]{imgs/smac/regd/qmix_regd0005_27m_vs_30m.pdf}
		\end{minipage}
	}}
	\caption{The performance of QMIX and QMIX-GRE.
	In (a)\emph{Lumberjacks} and (b)\emph{TrafficJunction10} from gridworld, QMIX is able to train a good joint policy, although with a large variance.
	GRE helps the algorithm to more stably achieve a good team policy.
	In (c)\emph{3s5z}, (d)\emph{MMM2} and (e)\emph{27m vs 30m} from \emph{SMAC}, QMIX-GRE speeds up the training and improves the overall performance.} 
	\label{qmix-GRE performance}
\end{figure*}

We test our method on both gridworld and several SMAC maps.
The results are shown in Figure~\ref{qmix-GRE performance}.
More results on SMAC can be found in appendix.
In terms of the overall performance, QMIX-GRE can outperform QMIX or at least achieve comparable performance.
In terms of training efficiency, QMIX-GRE has a significant advantage over QMIX in the early stage, indicating that QMIX-GRE can speed up the training process.
% We can find that with GRE, the performance of QMIX comparatively improves.
% In simple gridworld environments like Lumberjacks and TrafficJunction10, QMIX itself could already solve the task with a high test return, but with a large variation.
% In such envrionments, GRE helps to reduce the variance and maintain the performance.
% It can be seen that in these two environments the performance of QMIX drops at the middle stage in the training while QMIX-GRE does not.

In simple gridworld environments like Lumberjacks and TrafficJunction10, QMIX-GRE can achieve comparable performance.
In such a simple environment, QMIX itself can already solve tasks with high test return, so it is difficult to obtain further improvement.
However, QMIX drops at the middle stage in the training while QMIX-GRE improves the return gradually.
% For SMAC environments, QMIX-GRE can greatly boost the performance on the complex map,  like \emph{27m vs 30m}.
% Among the experimental maps in SMAC environments, \emph{27m vs 30m} is the most complex one that QMIX can only achieve 40\% win rate while the win rates of QMIX on \emph{3s5z} and \emph{MMM2} could reach over 60\%.
We can see that QMIX-GRE greatly boosts the performance and achieves similar performance on \emph{3s5z}.
On \emph{MMM2} and \emph{27m vs 30m}, QMIX-GRE not only speeds up training, but also improves the overall performance.
The results show that the gradient entropy regularization would be more beneficial to the complex environment.

% In maps like \emph{3s vs 5z} and \emph{3s5z} where QMIX is able to learn a good cooperative joint policy, GRE helps to speed up the training while the performance do not drop.
% In difficult maps like \emph{27m vs 30m} where it's hard for QMIX to improve its winning rate, GRE helps to improve the overall performance.

\begin{figure}[htb]
	\centering
	\subfigure{
		\begin{minipage}{0.35\textwidth} 
            \includegraphics[width=\textwidth]{imgs/smac/MMM2_reg.pdf}
		\end{minipage}
	}
	\caption{The entropy curve of QMIX and QMIX-GRE on \emph{MMM2} from \emph{SMAC}.
	The normalized entropy of QMIX-GRE significantly decreases, which implies the effectiveness of GRE.} 
	\label{qmix-GRE entropy}
\end{figure}

\subsection{Discriminability of QMIX-GRE: RQ3}
To further investigate whether gradient entropy regularization indeed helps QMIX improve the discriminability of credit assignment, we collect the normalized gradient entropy data in the whole training process and compare it with QMIX.

% In order to test the discriminability of credit assignment in QMIX-GRE, we also collect the normalized entropy data in the training process and compare it with QMIX.
Due to the page limit, we only plot the entropy curve of \emph{MMM2} in SMAC, as shown in Figure \ref{qmix-GRE entropy}.
We can find that in the random exploration stage in the training, there is actually little difference between the entropy of QMIX and QMIX-GRE.
As training progresses, the entropy of QMIX-GRE is significantly smaller than QMIX, which means that QMIX-GRE tends to realize a more discriminative credit assignment.
% However in the later stages, the entropy of QMIX-GRE is significantly smaller than QMIX, while still keeping at a reasonable value.
It is worth mentioning that the gradient entropy is not that too small, which mainly results from the trade off between the optimization of TD loss and regularization term.
% This means that with GRE, QMIX is able to more discriminatively assign credits to agents, which benefits the performance improvement.

